ComFusion: Personalized Subject Generation in Multiple Specific Scenes From Single Image

Recent advancements in personalizing text-to-image (T2I) diffusion models have shown the capability to generate images based on personalized visual concepts using a limited number of user-provided examples. However, these models often struggle with maintaining high visual fidelity, particularly in manipulating scenes as defined by textual inputs. Addressing this, we introduce ComFusion, a novel approach that leverages pretrained models generating composition of a few user-provided subject images and predefined-text scenes, effectively fusing visual-subject instances with textual-specific scenes, resulting in the generation of high-fidelity instances within diverse scenes. ComFusion integrates a class-scene prior preservation regularization, which leverages composites the subject class and scene-specific knowledge from pretrained models to enhance generation fidelity. Additionally, ComFusion uses coarse generated images, ensuring they align effectively with both the instance image and scene texts. Consequently, ComFusion maintains a delicate balance between capturing the essence of the subject and maintaining scene fidelity.Extensive evaluations of ComFusion against various baselines in T2I personalization have demonstrated its qualitative and quantitative superiority.

==> Sections/Tables/prior_prompt_length.tex <==
\begin{table}[!htp]
  \centering
  %\fontsize{8}{8}\selectfont
  % \caption{Ablation studies of each loss and alternative designs. Time represents the totoal training time on 1 A100 GPU.} 
  % \vspace{-8pt}
  \resizebox{0.9\columnwidth}{!} {
  \begin{tabular}{l|ccc}
\toprule 
Methods&  DINO ($\uparrow$)& CLIP-I ($\uparrow$)&  CLIP-T ($\uparrow$) \\
\midrule 
Real Images&\textit{0.795} & \textit{0.859}&N/A \\
\midrule
DreamBooth (Unseen)&0.607&0.735& 0.214 \\
Ours ($L=5$, Unseen)&0.613  & 0.737 &0.258  \\
Ours ($L=10$, Unseen)&0.617 &0.741  &  0.274  \\
Ours ($L=15$, Unseen)& 0.618 &  0.749 &  0.297 \\
\midrule
% DreamBooth &0.619&0.752& 0.229 & 491.8 \\
% \hline
% Ours ($L=5$)&0.686  &0.842  & 0.351  \\
% Ours ($L=10$)& 0.672 & 0.829 &  0.329  \\
% \hline
Ours (Only Instance)& 0.724 & 0.872 &  0.369  \\
Ours (Only Scene)& N/A & N/A &  0.378  \\
DreamBooth (Only Instance)& 0.638 &0.841  & 0.359   \\
DreamBooth (Only Scene)& N/A & N/A & 0.287   \\
\midrule
% Ours ($\lamda_C^S=1$)&  &  &  &  \\
% Ours ($\lamda_F^S=0.01$)&  &  &  &  \\
% Ours ($\lamda_F^I=0.01$)&  &  &  &  \\
Ours ($\lambda_C^S=10$)&0.619  &0.768  &  0.334  \\
Ours ($\lambda_C^S=0.1$)&0.669  & 0.826 &  0.296  \\
Ours ($\lambda_F^S=0.1$)&0.529  &0.638  &  0.351 \\
Ours ($\lambda_F^S=0.001$)&0.732  &0.851  &0.272    \\
Ours ($\lambda_F^I=0.1$)&0.715  &0.842  & 0.302   \\
Ours ($\lambda_F^I=0.001$)& 0.546 &0.672  & 0.341   \\
\midrule
Ours (Full-Fledged)& 0.658 & 0.814 & 0.321  \\
\bottomrule
\end{tabular}
}
\vspace{-16pt}
%   \vspace{0.1mm}
  \label{tab:prompt_length}
\end{table}




% \begin{table}[!htp]
%   \centering
%   %\fontsize{8}{8}\selectfont
%   \caption{Resutls on unseen sets.} 
%   \vspace{-8pt}
%   \resizebox{0.9\columnwidth}{!} {
%   \begin{tabular}{l|ccc}
% \toprule 
% Methods&  DINO ($\uparrow$)& CLIP-I ($\uparrow$)&  CLIP-T ($\uparrow$) \\
% \midrule 
% Real Images&\textit{0.795} & \textit{0.859}&N/A \\
% \midrule
% % DreamBooth &0.619&0.752& 0.229 & 491.8 \\
% % \hline
% % Ours ($L=5$)&0.686  &0.842  & 0.351  \\
% % Ours ($L=10$)& 0.672 & 0.829 &  0.329  \\
% % Ours ($L=5$)&0.686  &0.842  & 0.351  \\
% % Ours ($L=10$)& 0.672 & 0.829 &  0.329  \\
% % DreamBooth ($L=5$)&0.542  & 0.659& 0.237  \\
% % Ours ($L=5$)& 0.569 & 0.684& 0.259  \\
% % Ours ($L=10$)&0.595 &0.721  & 0.270   \\
% Ours ($L=5$)&0.613  & 0.737 &0.258  \\
% Ours ($L=10$)&0.620 &0.741  &  0.274  \\
% % DreamBooth ($L=10$)& 0.579& 0.712 &  0.212  \\
% % \hline
% % \hline
% % Ours ($\lamda_C^S=1$)&  &  &  &  \\
% % Ours ($\lamda_F^S=0.01$)&  &  &  &  \\
% % Ours ($\lamda_F^I=0.01$)&  &  &  &  \\
% % Ours ($\lambda_C^S=10$)&0.619  &0.768  &  0.334  \\
% % Ours ($\lambda_C^S=0.1$)&0.669  & 0.826 &  0.296  \\
% % Ours ($\lambda_F^S=0.1$)&0.529  &0.638  &  0.351 \\
% % Ours ($\lambda_F^S=0.001$)&0.732  &0.851  &0.272    \\
% % Ours ($\lambda_F^I=0.1$)&0.715  &0.842  & 0.302   \\
% % Ours ($\lambda_F^I=0.001$)& 0.546 &0.672  & 0.341   \\
% \midrule
% % Ours ($L=15$)& 0.658 & 0.814 & 0.321  \\
% DreamBooth&0.607&0.735& 0.214 \\
% Ours ($L=15$)& 0.618 &  0.749 &  0.297 \\
% \bottomrule
% \end{tabular}
% }

%   \vspace{0.1mm}
  % \label{tab:prompt_length_unseen}
% \end{table}


==> Sections/Tables/score_metric_supple.tex <==
\begin{table}[!htp]
  \centering
  %\fontsize{8}{8}\selectfont
  \caption{Ablation studies of each loss and alternative designs. Time represents the totoal training time on 1 A100 GPU.} 
  \vspace{-8pt}
  \resizebox{0.9\columnwidth}{!} {
  \begin{tabular}{l|ccc|c}
\toprule 
Methods&  DINO ($\uparrow$)& CLIP-I ($\uparrow$)&  CLIP-T ($\uparrow$) & Time(/s)\\
\midrule 
Real Images&\textit{0.795} & \textit{0.859}&N/A & N/A\\
\midrule
DreamBooth(5) &&&& \\
DreamBooth(3) &&&& \\
DreamBooth(1) &0.619&0.752& 0.229 & 491.8 \\

\hline
Ours (5)  &&&& \\
Ours (3)  &&&& \\
\midrule
Ours (1)& 0.658 & 0.814 & 0.321 & 597.7 \\
\bottomrule
\end{tabular}
}

%   \vspace{0.1mm}
  \label{tab:instance_num}
\end{table}


